Behavioral uncertainty quantification for data-driven control

This paper explores the problem of uncertainty quantification in the behavioral setting for data-driven control. Building on classical ideas from robust control, the problem is regarded as that of selecting a metric which is best suited to a data-based description of uncertainties. Leveraging on Willems' fundamental lemma, restricted behaviors are viewed as subspaces of fixed dimension, which may be represented by data matrices. Consequently, metrics between restricted behaviors are defined as distances between points on the Grassmannian, i.e., the set of all subspaces of equal dimension in a given vector space. A new metric is defined on the set of restricted behaviors as a direct finite-time counterpart of the classical gap metric. The metric is shown to capture parametric uncertainty for the class of autoregressive (AR) models. Numerical simulations illustrate the value of the new metric with a data-driven mode recognition and control case study.

==> refs.tex <==
@preamble{"\newcommand{\TAC}{\textit{{IEEE} Trans. Autom. Control}}" }
@preamble{"\newcommand{\TCST}{\textit{{IEEE} Trans. Syst. Tech.}}" }
@preamble{"\newcommand{\TIT}{\textit{{IEEE} Trans. Inform. Theory}}" }
@preamble{"\newcommand{\TSP}{\textit{{IEEE} Trans. Sign. Proc.}}" }
@preamble{"\newcommand{\SCL}{\textit{Syst. Control Lett.}}" }
@preamble{"\newcommand{\IJC}{\textit{Int. J. Control}}" }
@preamble{"\newcommand{\EJC}{\textit{Eur. J. Control}}" }
@preamble{"\newcommand{\ACC}{\textit{Proc. Amer. Control Conf.}}" }
@preamble{"\newcommand{\ECC}{\textit{Proc. Eur. Control Conf.}}" }
@preamble{"\newcommand{\CDC}[1]{\textit{Proc. {#1} Conf. Decision Control}}" }
@preamble{"\newcommand{\CDCs}[1]{\textit{{#1} Conf. Decision Control}}" }
@preamble{"\newcommand{\IFAC}[1]{\textit{Proc.  {#1}  IFAC World Congr.}}" }
@preamble{"\newcommand{\SIAM}{\textit{SIAM J. Control Optim.}}" } 
@preamble{"\newcommand{\MCSS}{\textit{Math. Control, Sign. Syst.}}" } 
@preamble{"\newcommand{\NOLCOS}[1]{\textit{Proc. {#1} IFAC Symp. Nonlinear Control Syst.}}"} 
@preamble{"\newcommand{\MTNS}[1]{\textit{ Proc. {#1} Math. Symp. Netw. Syst.}}"} 
 
 
@inproceedings{hong2014geodesic,
  title={Geodesic regression on the Grassmannian},
  author={Hong, Yi and Kwitt, Roland and Singh, Nikhil and Davis, Brad and Vasconcelos, Nuno and Niethammer, Marc},
  booktitle={Eur.  Conf.   Comp. Vision},
  pages={632--646},
  year={2014},
  organization={Springer}
}

@book{boothby2003introduction,
  title={An introduction to differentiable manifolds and Riemannian geometry (2nd Edition)},
  author={Boothby, W. M.},
  year={1986},
      address={London,  U. K.},
  publisher={{Academic Press}}
}




@book{VanOverschee1996subspace,
author = {{Van Overschee}, P. and {De Moor}, B.},
title = {{Subspace identification for linear systems: theory - implementation - applications}},
publisher={{Kluwer}},
address = {Dordrecht, The Netherlands},
year = {1996}
}

@book{ljung1999system,
  title={System identification - Theory for the user {(2nd edition)}},
  author={Ljung, L.},
  year={1999},
  address={Upper Saddle River, NJ, USA},
  publisher={Prentice-Hall}
}

@book{soderstrom1989system,
  title={System identification},
 author={S{\"o}derstr{\"o}m, T. D. and Stoica, P. G.},
  year={1989},
  address={Upper Saddle River, NJ, USA},
  publisher={Prentice-Hall}
} 
 

 @article{du2018robust,
  title={A robust algorithm for online switched system identification},
  author={Du, Zhe and Balzano, Laura and Ozay, Necmiye},
  journal={IFAC-PapersOnLine},
  volume={51},
  number={15},
  pages={293--298},
  year={2018},
  publisher={Elsevier}
}
 
@article{celi2022data,
  title={Data-driven Meets Geometric Control: Zero Dynamics, Subspace Stabilization, and Malicious Attacks},
  author={Celi, Federico and Pasqualetti, Fabio},
  journal={arXiv preprint arXiv:2201.03656},
  year={2022}
} 
 
 @book{kato1980perturbation,
  title={Perturbation theory for linear operators (2nd Edition)},
  author={Kato, T.},
  address={New York, NY, USA},
  year={1980},
  publisher={Springer}
}
 
 
@article{georgiou1990optimal,
  author={Georgiou, T.T.  and Smith, M.C.},
  journal={\TAC}, 
  title={Optimal robustness in the gap metric}, 
  year={1990},
  volume={35},
  number={6},
  pages={673-686},
  doi={10.1109/9.53546}
  } 
 
@article{ball2006equivalence,
  title={Equivalence of a behavioral distance and the gap metric},
  author={Ball, J.  A. and Sasane, A. J.},
  journal={\SCL},
  volume={55},
  number={3},
  pages={214--222},
  year={2006},
  publisher={Elsevier}
} 
 
@article{trentelman2013distance,
  title={Distance between behaviors and rational representations},
  author={Trentelman, H.  L and Gottimukkala, S. V.},
  journal={\SIAM },
  volume={51},
  number={6},
  pages={4211--4241},
  year={2013},
  publisher={SIAM}
} 
 
@article{absil2004riemannian,
  title={{Riemannian geometry of Grassmann manifolds with a view on algorithmic computation}},
  author={Absil, P. A. and Mahony, R. and Sepulchre, R.},
  journal={Acta Applicandae Mathematica},
  volume={80},
  number={2},
  pages={199--220},
  year={2004}
} 
 
@article{weinstein2000almost,
  title={Almost invariant submanifolds for compact group actions},
  author={Weinstein, A.},
  journal={J.   Eur.  Math.  Soc.},
  volume={2},
  number={1},
  pages={53--86},
  year={2000}
} 
 
@book{deza2009encyclopedia,
  title={Encyclopedia of distances},
  author={Deza, M.  M. and Deza, E.},
  address={New York, NY, USA},
  year={2009},
  publisher={Springer}
} 
 
@book{munkres2000topology,
  title={Topology (2nd Edition)},
  author={Munkres, J. R.},
  year={2000},
  address={Upper Saddle River, NJ, USA},
  publisher={Prentice Hall}
} 
 
@article{huang2021robust,
  title={Robust data-enabled predictive control: Tractable formulations and performance guarantees},
  author={Huang, L. and Zhen, J. and Lygeros, J. and D{\"o}rfler, F.},
  journal={arXiv preprint arXiv:2105.07199},
  year={2021}
} 
 
 @article{koenings2017data,
  title={{A data-driven computation method for the gap metric and the optimal stability margin}},
  author={Koenings, T.  and Krueger, M. and Luo, H. and Ding, S.  X.},
  journal={\TAC},
  volume={63},
  number={3},
  pages={805--810},
  year={2017},
  publisher={IEEE}
}

 
 @book{vidyasagar2011control,
  title={{Control System Synthesis: A Factorization Approach, Part II}},
  author={Vidyasagar, M.},
  year={2011},
    address={London,  U. K.},
  publisher={Morgan \& Claypool Publishers}
}
 
 
 
@book{willems1971analysis,
  title={The analysis of feedback systems},
  author={Willems, J. C.},
  year={1971},
  address={London,  U. K.},
  publisher={MIT Press}
}
 
@book{partington2004linear,
  title={{Linear operators and linear systems: an analytical approach to control theory}},
  author={Partington, J. R.},
  address={Cambridge,  U. K.},
  year={2004},
  publisher={Cambridge Univ. Press}
} 


@book{antoulas2005approximation,
   title = {Approximation of large-scale dynamical systems},
   author = {Antoulas, A. C.},
   publisher = {SIAM},
   address = {Philadelphia, PA, USA},
   year = {2005}
}
 
@book{carothers2000real,
  title={Real analysis},
  author={Carothers, N. L.},
  year={2000},
    address={Cambridge,  U. K.},
  publisher={Cambridge Univ. Press}
} 
 
@article{dorfler2022bridging,
  title={{Bridging direct \& indirect data-driven control formulations via regularizations and relaxations}},
  author={Dorfler, F. and Coulson, J. and Markovsky, I.},
  journal={\TAC},
  year={2022},
  publisher={IEEE}
} 
 
 @article{qui1992pointwise,
  title={Pointwise gap metrics on transfer matrices},
  author={Qui, L. and Davison, E. J.},
  journal={\TAC},
  volume={37},
  number={6},
  pages={741--758},
  year={1992}
}
 

@book{golub2013matrix,
  title={Matrix computations (4th Ed.)},
  author={Golub, G. H. and Van Loan, C. F.},
  year={2013},
  address={Baltimore, MD, USA},
  publisher={Johns Hopkins Univ. Press}
} 
 
@book{stewart1990perturbation,
  title={{Matrix Perturbation Theory}},
  author={Stewart, G.W.  and Sun, J.G.},
  year={1990},
  publisher={Academic Press},
  address={New York, NY, USA}  
} 
 
@book{doyle1992feedback,
  title={Feedback control theory},
  author={Doyle, J. C.  and Francis, B. A.  and Tannenbaum, A. R.},
  year={1992},
    address={New York, NY, USA} ,
  publisher={Macmillan}
}

 
@book{zhou1996robust,
  title={Robust and optimal control},
  author={Zhou, K. and Doyle, J. C. and Glover, K.},
  address={New Jersey, NJ, USA},
  year={1996},
  publisher={Prentice Hall}
}   
 
@book{vinnicombe2001uncertainty,
  title={{Uncertainty and feedback: $H_{\infty}$ loop-shaping and the $\nu$-gap metric}},
  author={Vinnicombe, G.},
  year={2001},
  address={London,  U.K.},
  publisher={Imperial College Press}
}
 
@article{trentelman2013distance,
  title={Distance between behaviors and rational representations},
  author={Trentelman, Harry L and Gottimukkala, Sasanka V},
  journal={\SIAM},
  volume={51},
  number={6},
  pages={4211--4241},
  year={2013}
} 
 
@article{sasane2003distance,
  title={Distance between behaviours},
  author={Sasane, A. J.},
  journal={\IJC},
  volume={76},
  number={12},
  pages={1214--1223},
  year={2003}
} 
 
@article{ball2006equivalence,
  title={Equivalence of a behavioral distance and the gap metric},
  author={Ball, J.  A. and Sasane, A. J.},
  journal={\SCL},
  volume={55},
  number={3},
  pages={214--222},
  year={2006}
} 
 
@inproceedings{berberich2020robust,
  title={Robust data-driven state-feedback design},
  author={Berberich, J.  and Koch, A.  and Scherer, C. W and Allg{\"o}wer, F.},
  booktitle={\ACC},
   address={Denver, CO, USA},
  pages={1532--1538},
  year={2020}
}
 
@article{bisoffi2021data,
  title={{Data-driven control via Petersen's lemma}},
  author={Bisoffi, A. and De Persis, C. and Tesi, P.},
  journal={arXiv:2109.12175},
  year={2021}
} 
 
@article{van2021matrix,
  title={A Matrix Finsler's Lemma with Applications to Data-Driven Control},
  author={van Waarde, H.  J. and Camlibel,  M. K.},
  journal={arXiv:2103.13461},
  year={2021}
} 
 
@inproceedings{xue2021data,
  title={Data-driven system level synthesis},
  author={Xue, A.  and Matni, N.},
  booktitle={Learning for Dynamics and Control},
  pages={189--200},
  year={2021},
  organization={PMLR}
} 
 
@inproceedings{yin2021low,
  title={On Low-Rank Hankel Matrix Denoising},
  author={Yin, M. and Smith, R. S.},
   booktitle={19th IFAC Symp.  Syst.  Identif.},
  pages={198--203},
   address={Padova, Italy},
  year={2019}
} 
 
@inproceedings{huang2019data,
  title={Data-enabled predictive control for grid-connected power converters},
  author={Huang, Linbin and Coulson, Jeremy and Lygeros, John and D{\"o}rfler, Florian},
  booktitle={\CDC{58th}},
  pages={8130--8135},
    address={Naples, Italy},
  year={2019}
} 
 
@inproceedings{carlet2020data,
  title={Data-driven predictive current control for synchronous motor drives},
  author={Carlet, P.  G. and Favato, A. and Bolognani, S. and D{\"o}rfler, F.},
  booktitle={IEEE Energy Conversion Congress and Exposition},
  pages={5148--5154},
  year={2020},
    address={Detroit, MI, USA}
} 
 
@article{coulson2021distributionally,
  title={Distributionally robust chance constrained data-enabled predictive control},
  author={Coulson,  J.  and Lygeros, J. and D{\"o}rfler, F.},
    journal={\TAC},
  year={2021},
  publisher={IEEE}
} 
 
@article{de2019formulas,
  title={Formulas for data-driven control: Stabilization, optimality, and robustness},
  author={De Persis, C.  and Tesi, P.},
  journal={\TAC},
  volume={65},
  number={3},
  pages={909--924},
  year={2019},
  publisher={IEEE}
} 
 
@inproceedings{coulson2019data,
  title={Data-enabled predictive control: In the shallows of the DeePC},
  author={Coulson,  J.  and Lygeros, J. and D{\"o}rfler, F.},
  booktitle={\ECC},
  pages={307--312},
  address={Naples, Italy},
  year={2019}
} 
 
@article{markovsky2021behavioral,
  title={Behavioral systems theory in data-driven analysis, signal processing, and control},
  author={Markovsky,  I. and D{\"o}rfler, F.},
  journal={Ann.  Rev.  Control},
  volume={52},
  pages={42--64},
  year={2021}
} 
 
@book{doob1953stochastic,
  title={Stochastic processes},
  author={Doob, J. L.},
  address={New York, NY, USA},
  year={1953},
  publisher={John Wiley \& Sons}
} 
 
@book{bishop2006pattern,
  title={Pattern recognition and machine learning},
  author={Bishop, C.  M. },
  address={New York,  NY,  USA},
  year={2006},
  publisher={Springer}
} 
 
@book{luenberger1969optimization,
  title={Optimization by vector space methods},
  author={Luenberger, David G},
  year={1969},
  address={New York,  NY,  USA},
    publisher={John Wiley \& Sons}
} 
 
@book{hamming1962numerical,
  title={Numerical methods for scientists and engineers},
  author={Hamming, R.},
    year={1962},
     address={New York,  NY,  USA},
  publisher={McGraw-Hill}
} 
 
@book{widrow1985adaptive,
  title={Adaptive Signal Processing},
  author={Widrow, B.  and Stearns, S. D.},
  year={1985},
     address={Englewood Cliffs, NJ,  USA},
  publisher={Prentice-Hall}
} 
  
 
@book{kantz2004nonlinear,
  title={Nonlinear time series analysis},
  author={Kantz, H. and Schreiber, T.},
  year={2004},
     address={Cambridge,  U.K.},
  publisher={Cambridge Univ.  Press}
} 
 
 @book{hamilton1994time,
  title={Time series analysis},
  author={Hamilton, James Douglas},
  year={1994},
   address={Princeton, NJ, USA},
  publisher={Princeton Univ.  Press}
}

@article{kalman1960new,
  title={A new approach to linear filtering and prediction problems},
  author={Kalman, R.  E.},
	  journal={Trans.  ASME J.  Basic Eng.},
  volume={82},
  number={1},
  pages={35--45},
  year={1960}
}



@book{wiener1949extrapolation,
  title={The Extrapolation, Interpolation and Smoothing of Stationary Time Series},
  author={Wiener, N. },
     year={1949},
 address={New York, NY, USA},
  publisher={John Wiley \& Sons}
}

@inproceedings{zames1981uncertainty,
  title={Uncertainty in unstable systems: The gap metric},
  author={Zames, G. and El-Sakkary,  A.},
  booktitle={\IFAC{8th}}, 
  volume={14},
  number={2},
  pages={149--152},
  year={1981},
}



@book{astrom1995adaptive,
  title={Adaptive control (2nd edition)},
  author={{\AA}str{\"o}m, K. J. and Wittenmark, B.},
 year={1995},
 address={Reading, MA, USA},
  publisher={Addison-Wesley}
}


@book{sastry1989adaptive,
  title={Adaptive control: stability, convergence and robustness},
  author={Sastry, S. and Bodson, M.},
  year={1989},
  address={ Englewood Cliffs, NJ, USA},
  publisher={Prentice-Hall}
}


@book{ljung1999system,
  title={System identification - Theory for the user {(2nd edition)}},
  author={Ljung, L.},
  year={1999},
  address={Upper Saddle River, NJ, USA},
  publisher={Prentice-Hall}
}
 


@book{VanOverschee1996subspace,
author = {{Van Overschee}, P. and {De Moor}, B.},
title = {{Subspace identification for linear systems: theory - implementation - applications}},
publisher={{Kluwer}},
address = {Dordrecht, The Netherlands},
year = {1996}
}

@article{ye2016schubert,
  title={Schubert varieties and distances between subspaces of different dimensions},
  author={Ye,  K. and Lim, L.  H.},
  journal={SIAM J.   Mat.  Anal.  Appl.},
  volume={37},
  number={3},
  pages={1176--1197},
  year={2016}
}

@article{wong1967differential,
  title={Differential geometry of Grassmann manifolds},
  author={Wong, Y.  C.},
  journal={Proc.  Nat.  Acad.  Sci.  USA},
  volume={57},
  number={3},
  pages={589},
  year={1967}
}

@book{absil2009optimization,
  title={Optimization algorithms on matrix manifolds},
  author={Absil, P. A. and Mahony, R. and Sepulchre, R.},
  year={2009},
  address = {Princeton, NJ, USA},
  publisher={Princeton Univ. Press}
}

@article{markovsky2020identifiability,
  title={Identifiability in the behavioral setting},
  author={Markovsky, Ivan and D{\"o}rfler, Florian},
  journal={Vrije Universiteit Brussel, Tech. Rep},
  year={2020},
  url={{http://homepages.vub.ac.be/~imarkovs/publications/identifiability.pdf.}}
}

@article{willems1986time,
  title={{From time series to linear system—Part I. Finite dimensional linear time invariant systems}},
  author={Willems, J. C.},
  journal={Automatica},
  volume={22},
  number={5},
  pages={561--580},
  year={1986}
}

@book{willems1997introduction,
  title={Introduction to mathematical systems theory: a behavioral approach},
  author={Willems,  J.  C.  and Polderman,  J.  W.},
    address={New York, NY, USA},
  year={1997},
  publisher={Springer}
}

@article{willems2007behavioral,
  title={The behavioral approach to open and interconnected systems},
  author={Willems,  J.  C.},
  journal={IEEE Control Syst.  Mag.},
  volume={27},
  number={6},
  pages={46--99},
  year={2007},
  publisher={IEEE}
}



@article{willems2005note,
  title={A note on persistency of excitation},
  author={Willems, J. C. and Rapisarda, P. and Markovsky, I. and De Moor, B. L. M.},
  journal={\SCL},
  volume={54},
  number={4},
  pages={325--329},
  year={2005},
  publisher={Elsevier}
}

 
@article{van2020willems,
  title={Willems’ fundamental lemma for state-space systems and its extension to multiple datasets},
  author={van Waarde, H. J. and De Persis, C. and Camlibel, M. K. and Tesi, P.},
  journal={IEEE Control Systems Letters},
  volume={4},
  number={3},
  pages={602--607},
  year={2020}
}
 


@ARTICLE{vanWaarde2020, 
author={H. J. {van Waarde} and J. {Eising} and H. L. {Trentelman} and M. K. {Camlibel}}, journal={IEEE Transactions on Automatic Control}, 
title={Data informativity: a new perspective on data-driven analysis and control}, 
year={2020}, 
  volume={65},
  number={11},
  pages={4753--4768}
}

@ARTICLE{vanWaarde2022,
  author={van Waarde, H. J. and Camlibel, M. K. and Mesbahi, M.},
  journal={IEEE Transactions on Automatic Control}, 
  title={From Noisy Data to Feedback Controllers: Nonconservative Design via a Matrix {S}-Lemma}, 
  year={2022},
  volume={67},
  number={1},
  pages={162--175}
  }
